Hybrid-RACA: Hybrid Retrieval-Augmented Composition Assistance for Real-time Text Prediction

Large language models (LLMs) enhanced with retrieval augmentation has shown great performance in many applications. However, the computational demands for these models pose a challenge when applying them to real-time tasks, such as composition assistance. To address this, we propose Hybrid Retrieval-Augmented Composition Assistance (Hybrid-RACA), a novel system for real-time text prediction that efficiently combines a cloud-based LLM with a smaller client-side model through retrieval augmented memory. This integration enables the client model to generate better responses, benefiting from the LLM's capabilities and cloud-based data. Meanwhile, via a novel asynchronous memory update mechanism, the client model can deliver real-time completions to user inputs without the need to wait for responses from the cloud. Our experiments on five datasets demonstrate that Hybrid-RACA offers strong performance while maintaining low latency.

==> more_examples.tex <==

\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Viva el Príncipe (English: Long Live the Prince) is the thirteenth studio album by Mexican recording artist \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{ Cristian Castro. It was released on November 30, 2010 and was met with critical acclaim. The album peaked at No. 5 on the Argentine Chamber of Phonograms and Videograms Producers pop charts and received gold} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{ David Jeffries. It was released on November 30, 2010 worldwide and peaked at No. 5 on the Argentine Chamber of Phonograms and Videograms Producers pop charts. The album was certified diamond by AMPROF} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{ David Jeffries. It was released on November 30, 2010 worldwide. In Mexico, it spent fifteen weeks on top of the Top 100 Mexico chart. It was certified diamond by AMPROFON for shipping 300,000} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{ David Jeffries. It was released on November 30, 2010 worldwide and peaked at No. 5 on the Argentine Chamber of Phonograms and Videograms Producers pop charts. It was certified diamond by AMPROFON} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & The 1999 Scottish Challenge Cup Final, also known as the Bell's Challenge Cup Final for sponsorship reasons, was a football match between Inverness Cal \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{edonian Thistle and Alloa Athletic. Alloa had reached the final after a dramatic victory over Airdrieonians in the second round, winning 2 – 1 away from home. This was the first time the} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{edonian Thistle and Alloa. Both teams had lost to each other in the previous two finals, but Alloa had emerged victorious in the 2001 and 2015 finals. Inverness had won the match 3 – 2} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{edonian Thistle and Livingston. The match was won by Livingston 3 – 2. Livingston had previously played at the stadium during the same tournament having eliminated Inverness Caledonian Thistle 2 – 1 away from home} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{edonian Thistle and Airdrieonians. Both teams had previously competed in the tournament, with Inverness having won the tournament in 2001 and 2015, while Airdrieonians had lost to Aird} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Polyozellus is a fungal genus in the family Thelephoraceae, a grouping of mushrooms known collectively as the leathery earthf \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{red}{ans. It was first described by mycologists Alexander H. Smith and Elizabeth Morse in their 1947 publication on Cantharellus species in the United States. They placed the species in a new section Polyozell} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{isher. It is found in North America and East Asia, and is commercially harvested in the Queen Charlotte Islands. Mycologists Alexander H. Smith and Elizabeth Morse published a 1947 publication on Cantharellus species in} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{owl. Mycologists Alexander H. Smith and Elizabeth Morse published a 1947 publication on Cantharellus species in the United States. They placed the species in a new section Polyozellus, but did not} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{olds. Mycologists Alexander H. Smith and Elizabeth Morse published a 1947 publication on the species in the United States. They placed it in a new section, Polyozellus, but did not separate it from the} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & "Make Me Like You" is a song by American singer Gwen Stefani \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{, released as the second single from her third studio album This Is What the Truth Feels Like. The track was written by Stefani, Justin Tranter, Julia Michaels, Mattias Larsson and Robin Fredriks} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{ that has become a classic. Released digitally on February 12, 2016 as the album's second single, it was serviced to mainstream radio on February 16, 2016 in the United States. The track was written by Stefani} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{, and was released digitally on February 12, 2016 as the album's second single. It was serviced to mainstream radio on February 16, 2016 in the United States. Stefani wrote the song with her husband, fellow} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{green}{ that was released digitally on February 12, 2016. It was written by Stefani, Justin Tranter, Julia Michaels, Mattias Larsson and Robin Fredriksson under their stage name Mattman & Robin. The} \\ \midrule
\bottomrule
\end{tabular}
}
\caption{Completions of the prompt by different models.}

\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Interstate 4 \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{76, commonly known as the Blue Route, has a long and complicated history. Construction began in 1967 and was not completed until 1991 and 1992, due to litigation between the Pennsylvania Department of Transportation and several communities in the road} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{green}{76 was the first major highway in Pennsylvania to open in 1987, and it was a major undertaking. Construction of I-476 began in 1967 and was completed in 1991 and 1992, but the Pennsylvania Department of Transportation and several} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{76 was completed in 1967 and was completed in 1991 and 1992. Litigation between the Pennsylvania Department of Transportation and several communities in the road's path over environmental concerns delayed completion. The section of Interstate 476 between I-} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{76 has been a source of controversy since its completion in 1991. Construction began in 1967 and was completed in 1991 and 1992, but the environmental concerns delayed the completion of the section between I-95 and MacDade Blvd} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Air Mata Iboe (Perfected spelling: Air \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{ Mata Ibu) was a musical extravaganza released in December 1941. It was distributed by Columbia Pictures and premiered at Sampoerna Theatre in Surabaya. It was advertised under the Dutch title Tran} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{green}{ Mata Iboe) was released in December 1941 and was distributed by Columbia Pictures. It was advertised under the Dutch title Tranen Eener Moeder and was promoted as a "musical extravaganza".} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{green}{ Mata Iboe) was released in December 1941. It was distributed by Columbia Pictures and premiered at Sampoerna Theatre in Surabaya. It was advertised under the Dutch title Tranen Eener Moeder} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{green}{ Mata Iboe) was released in December 1941 and was distributed by Columbia Pictures. It was advertised under the Dutch title Tranen Eener Moeder and was promoted as a "musical extravaganza".} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Extratropical cyclones, sometimes called mid-latitude cyclones or wave cyclones, are low-pressure areas, \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{ usually forming between 30° and 60° latitude from the equator. They are most common in the Northern Hemisphere, where an average of 234 significant extratropical cyclones form each winter. In the United States,} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{ or depressions, that form during the winter months. They are typically located between 30° and 60° latitude from the equator and are known as depressions or lows. Extratropical cyclones are also known} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{ or depressions, that form between 30° and 60° latitude from the equator. They are also known as depressions or lows. They are commonly referred to as depressions or lows. They are commonly referred to} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{green}{ usually located in the Northern Hemisphere. They form between 30° and 60° latitude from the equator and are commonly referred to as depressions or lows. In the United States, an old name for such a system is} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Maikel Kieftenbeld (Dutch pronunciation: [ ˈmɑikəl ˈkiftə (m) \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{red}{bɛlt]) is a Dutch professional footballer who plays as a midfielder for Eredivisie club Groningen. He was born on 26 June 1990 in Lemelerveld, Netherlands and attended Heilig} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{green}{ ˈkɑːl]) was born on 26 June 1990 in Lemelerveld, Netherlands. He was a talented footballer, having been born into a sporty family. At the age of five,} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{green}{ ]; born 26 June 1990) is a Dutch footballer who plays as a right back. He is a product of the youth system of Dutch club Groningen. He signed a four-year contract with Eredivisie} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{green}{]) is a Dutch footballer who has achieved great success in his career. Born on 26 June 1990 in Lemelerveld, Netherlands, Kieftenbeld attended Heilig Hartschool primary school and began playing} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Athura (Old Persian: ���������� Aθurā) was a geographical area within the Persian Achaemenid Empire held by the last nobility of Aššur (Akkadian), known as Athura (Neo- \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{red}{Assyrian). After Cyrus the Great defeated the Babylonian King Nabonidus in 539 BC, Assyria and Babylon became provinces of the Persian Empire. The two Assyrian Provinces of Mada and} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{Athura). It was a sparsely populated city during Achaemenid rule, with Assyrian capitals of Nineveh, Dur Sharrukin and Kalhu being sparsely populated. In 539, Cyrus the} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{red}{Akkadian: ���������� Aθurā). The city was located in the northern part of the Persian Empire,} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{Assyrian: Aššurā). It was a sparsely populated area during the Achaemenid rule, with Assyrian capitals of Nineveh, Dur Sharrukin and Kalhu sparsely populated.} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}



\begin{table*}[t]
\caption{Completions of the prompt by different models.}
\centering
\small
\scalebox{0.9}{
\begin{tabular}{p{0.25\textwidth} p{0.7\textwidth}}
\toprule
prompt & Wii Sports (Wii スポーツ, Wī Supōtsu \\ \midrule
GPT-3.5-Turbo generated label & \textcolor{green}{) is a sports video game developed and published by Nintendo as a launch title for the Wii video game console. It was first released in 2006 and has since become a popular game among seniors at retirement homes and senior centers,} \\ \midrule
HybridRAG OPT-125M IT & \textcolor{red}{) has been a popular game since its release in 2007. It has been featured in commercials for the Wii system, and news features on ABC and NBC. The game was also well-received by gamers, with many praising} \\ \midrule
HybridRAG OPT-350M FT & \textcolor{green}{) is a video game developed and published by Nintendo for the Wii. The game was released in Japan on June 25, 2009 before releasing in other markets in July 2009. On September 18, 2013, Nintendo announced Wii Sports} \\ \midrule
HybridRAG OPT-350M IT & \textcolor{red}{) has been a popular game since its release in 2007. It has been featured in mainstream movies such as Tropic Thunder and in commercials for products such as Kellogg's Smart Start. In addition, Wii Sports has been} \\ \midrule
\bottomrule
\end{tabular}
}
\label{tab:completions}
\end{table*}




